Balanced-Viscosity solutions for multi-rate systems

Several mechanical systems are modeled by the static momentum balance for the displacement $u$ coupled with a rate-independent flow rule for some internal variable $z$. We consider a class of abstract systems of ODEs which have the same structure, albeit in a finite-dimensional setting, and regularize both the static equation and the rate-independent flow rule by adding viscous dissipation terms with coefficients $\varepsilon^\alpha$ and $\varepsilon$, where $0<\varepsilon \ll 1$ and $\alpha>0$ is a fixed parameter. Therefore for $\alpha \neq 1$ $u$ and $z$ have different relaxation rates. We address the vanishing-viscosity analysis as $\varepsilon \downarrow 0$ of the viscous system. We prove that, up to a subsequence, (reparameterized) viscous solutions converge to a parameterized curve yielding a Balanced Viscosity solution to the original rate-independent system, and providing an accurate description of the system behavior at jumps. We also give a reformulation of the notion of Balanced Viscosity solution in terms of a system of subdifferential inclusions, showing that the viscosity in $u$ and the one in $z$ are involved in the jump dynamics in different ways, according to whether $\alpha>1$, $\alpha=1$, and $\alpha \in (0,1)$.

==> macro.tex <==
\newcommand{\quoderatdemonstrandum}{~\vrule height5pt depth0pt width5pt}

\newcommand{\N}{\mathbb{N}} % natural numbers
\newcommand{\R}{\mathbb{R}} % real numbers
\newcommand{\calA}{\mathcal{A}}
\newcommand{\teta}{\vartheta}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\eps}{\varepsilon}
\newcommand{\sfxx}{{\bm{\mathsf{x}}}}
\newcommand{\sfyy}{{\bm{\mathsf{y}}}}
\newcommand{\weaksto}{{\rightharpoonup^*}\,}
\newcommand{\weakto}{\rightharpoonup}
\newcommand{\Restr}[1]{\lower2pt\hbox{$|_{#1}$}}
\newcommand{\argmin}{\mathop{\mathrm{Argmin}}}
\newcommand{\DualDiss}{\Psi_0^*}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\ene}[2]{\mathcal{E}_{#1}(#2)}
\newcommand{\Varname}[1]{{\mathrm{Var}}_{#1}}
\newcommand{\pVarname}[1]{\text{\slshape Var}_{#1}}
\newcommand{\Var}[4]{\mathop{\mathrm{Var}}\nolimits_{#1}(#2;[#3,#4])}
\newcommand{\pVar}[4]{\mathop{\text{\slshape Var}}\nolimits_{#1}(#2;[#3,#4])}
\newcommand{\JVar}[4]{{\mathrm{Jmp}}_{#1}(#2;[#3,#4])}
\newcommand{\BV}{\mathrm{BV}}
\newcommand{\AC}{\mathrm{AC}}
\newcommand{\Finsl}[4]{{\mathfrak P}(\dot{#1}(#4),\dot{#2}(#4);#3,-\rmD\ene{#1(#4)}{#2(#4)})}
\newcommand{\vvm}[3]{\mathfrak{P}_{#1}({#2},{#3})}
\newcommand{\vvmV}[3]{\mathfrak{P}_\V({#3}; -\frsub \cE_{#1}({#2}))}
\newcommand{\vvmname}{\mathfrak{P}}
\newcommand{\vvmVname}{\mathfrak{P}_\V}
\newcommand{\vvmfulleps}[5]{\mathcal{P}_\eps({#1};{#4}; -\frsub \cE_{#2}({#3});{#5})}
\newcommand{\vvmfull}[5]{\mathcal{P}({#1};{#4}; -\frsub \cE_{#2}({#3});{#5})}
\newcommand{\vvmfullV}[5]{\mathcal{P}_\V({#1};{#4}; -\frsub \cE_{#2}({#3});{#5})}
\newcommand{\vvmfullepsname}{\mathcal{P}_\eps}
\newcommand{\vvmfullname}{\mathcal{P}}
\newcommand{\vvmfullVname}{\mathcal{P}_\V}
\newcommand{\Norm}[3]{\cB_{#3}\left(#1;#2\right)}
\newcommand{\FNorm}[3]{\mathcal{R}_{#3}\!\left(#1;#2\right)}
\newcommand{\Leb}[1]{\mathscr{L}^{#1}}
\newcommand{\topref}[2]{\stackrel{\eqref{#1}}#2}
\newcommand{\Contact}[1]{\Sigma_{#1}}
\newcommand{\VRIS}{\ensuremath{(\R,\mathcal{E},{\mathfrak P})}}
\newcommand{\PVRIS}{\ensuremath{(X,\mathcal{E},{\mathfrak P})}}
\newcommand{\RIS}{\ensuremath{(\B, \V,\mathcal{E}, \Diss{\B}{0}, \Diss{V}{})}}
\newcommand{\Mint}[4]{\int_{#1}^{#2}\mathrm{d}#3(#4)}
\newcommand{\Ibip}{$\mathfrak p$}
\newcommand{\bptname}{\mathfrak{p}}
\newcommand{\bpt}[2]{\mathfrak p(#1,#2)}
\newcommand{\IBip}{$\mathfrak P$}
\newcommand{\cost}[3]{\Delta_{#1}(#2,#3)}
\newcommand{\Cost}[4]{\Delta_{#1}(#2;#3,#4)}
\newcommand{\Dist}[3]{\Delta_{\cB_{#3}}(#1,#2)}
\newcommand{\FDist}[3]{\Delta_{\mathcal{R}_{#3}}(#1,#2)}
\newcommand{\bipcE}{{\mathfrak p,\mathcal{E}}}
\newcommand{\MU}[2]{\mu_{#1,#2}}
\newcommand{\essJ}{\mathop{\text{\upshape ess-J}}\nolimits}
\newcommand{\fnorm}[1]{\|#1\|}
\newcommand{\snorm}[1]{|#1|}
\newcommand{\dist}{\mathrm{dist}_*}
\newcommand{\taueps}{{\tau,\eps}}
\newcommand{\av}{``}
\newcommand{\candidu}{\bar{u}}
\newcommand{\qincrmin}[2]{q^-(#1;#2)}
\newcommand{\qincrplu}[2]{q^+(#1;#2)}
\newcommand{\qdecrmin}[2]{q_-(#1;#2)}
\newcommand{\qdecrplu}[2]{q_+(#1;#2)}
\newcommand{\foraa}{\text{for a.a.\,}}
\newcommand{\forae}{\text{for a.a.\,}}
\newcommand{\down}{\downarrow}
\newcommand{\up}{\uparrow}
\newcommand{\Banach}{B}
\newcommand{\Vanach}{V}
\newcommand{\V}{\Vanach}
\newcommand{\B}{\Banach}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\DDD}[3]{\begin{array}[t]{c}#1\vspace*{-1em}\\_{#2}\vspace*{-.5em}\\_{#3}\end{array}}
\newcommand{\ddd}[3]{\DDD{\begin{array}[t]{c}\underbrace{#1}\vspace*{.6em}\end{array}}{\text{\footnotesize #2}}{\text{\footnotesize #3}}}
%%%%%%%%%%%%% MACROS FOR INTERPOLANTS

\newcommand{\Utau}[1]{\mathrm{U}_\tau^{#1}}
\newcommand{\UU}{\mathrm{U}}
\newcommand{\piecewiseConstant}[2]{\overline{#1}_{\kern-1pt#2}}
\newcommand{\pwC}{\piecewiseConstant}
\newcommand{\underpiecewiseConstant}[2]{\underline{#1}_{\kern-1pt#2}}
\newcommand{\upwC}{\underpiecewiseConstant}


%\newcommand{\pwcr}{\underline{#1}_{\kern-1pt#2}}
%%
%%
\newcommand{\piecewiseLinear}[2]{#1_{\kern-1pt#2}}
\newcommand{\pwL}{\piecewiseLinear}
\newcommand{\pwM}[2]{\widetilde{#1}_{\kern-1pt#2}}
 \def\trait #1 #2 #3 {\vrule width #1pt height #2pt depth #3pt}

%%%%% MACROS FOR PARAMETRIZED SOLUTIONS

  \newcommand{\parat}{\mathsf{t}}
\newcommand{\parau}{\mathsf{u}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\para}{parametrized}
%%%%%%%%%%%% DISSIPATION FUNCTIONALS

\newcommand{\Diss}[2]{\Psi_{#1}^{#2}}
\newcommand{\Bnorm}[1]{\left|{#1}\right|}
\newcommand{\Vnorm}[1]{\left\|{#1}\right\|}
\newcommand{\Dis}{\Psi}
\newcommand{\pairing}[4]{ \sideset{_{#1 }}{_{ #2}}  {\mathop{\langle #3 , #4  \rangle}}}
\newcommand{\prods}[2]{\left(#1 , #2\right)_\V}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cg}[1]{\mathcal{G}(#1)}
\newcommand{\domainenergy}{D}
\newcommand{\frsub}{\partial}
\newcommand{\Dtau}{\Delta}
\newcommand{\ue}{u_\eps}
\newcommand{\ve}{v_\eps}
\newcommand{\sublev}[1]{\domainenergy_{#1}}
%%%%%%%%%%%%%%%%%%%% TO HIGHLIGHT CHANGES  and comments %%%%%%%%%


\newenvironment{rcomm}{\color{ddcyan} \textsf{R:} }{\color{black}}
\newenvironment{nrcomm}{\color{ddmagenta} \textsf{New R:} }{\color{black}}
\newenvironment{gcomm}{\color{red} \textsf{G:} }{\color{black}}
%\newenvironment{new}{\color{ddcyan}}{\color{black}}

